OmniEdit: Building Image Editing Generalist Models Through Specialist Supervision

Instruction-guided image editing methods have demonstrated significant potential by training diffusion models on automatically synthesized or manually annotated image editing pairs. However, these methods remain far from practical, real-life applications. We identify three primary challenges contributing to this gap. Firstly, existing models have limited editing skills due to the biased synthesis process. Secondly, these methods are trained with datasets with a high volume of noise and artifacts. This is due to the application of simple filtering methods like CLIP-score. Thirdly, all these datasets are restricted to a single low resolution and fixed aspect ratio, limiting the versatility to handle real-world use cases. In this paper, we present \omniedit, which is an omnipotent editor to handle seven different image editing tasks with any aspect ratio seamlessly. Our contribution is in four folds: (1) \omniedit is trained by utilizing the supervision from seven different specialist models to ensure task coverage. (2) we utilize importance sampling based on the scores provided by large multimodal models (like GPT-4o) instead of CLIP-score to improve the data quality. (3) we propose a new editing architecture called EditNet to greatly boost the editing success rate, (4) we provide images with different aspect ratios to ensure that our model can handle any image in the wild. We have curated a test set containing images of different aspect ratios, accompanied by diverse instructions to cover different tasks. Both automatic evaluation and human evaluations demonstrate that \omniedit can significantly outperform all the existing models. Our code, dataset and model will be available at https://tiger-ai-lab.github.io/OmniEdit/

==> section/x1_contribution.tex <==
\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

==> section/x2_acknowledgment.tex <==
\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

==> table/main/methods_comparison.tex <==
% \begin{wraptable}{r}{0.7\textwidth}
\definecolor{darkgreen}{rgb}{0.0, 0.8, 0.0}
\definecolor{darkred}{rgb}{0.8, 0.0, 0.0}
\begin{table}[h]
\centering
\caption{Comparison with different video editing methods and the type of editing tasks.}
\small
\def\arraystretch{1.0}
\setlength\tabcolsep{2 pt}
\scalebox{0.8}{
\begin{tabular}{lcccccc}
\toprule
\textbf{Method}        & \textbf{\begin{tabular}[c]{@{}c@{}}Prompt-based\\ Editing\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Reference-based\\ Style Transfer\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Subject-Driven\\ Editing\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Identity\\ Manipulation\end{tabular}} & \textbf{Tuning-Free?} & \textbf{Backbone}     \\
\midrule
Tune-A-Video~\citep{wu2023tune} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & Stable Diffusion \\ 
Pix2Video~\citep{ceylan2023pix2video} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkgreen}{\ding{51}} & SD-Depth \\ 
Gen-1~\citep{esser2023structure} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & Stable Diffusion \\ 
TokenFlow~\citep{tokenflow2023} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkgreen}{\ding{51}} & Stable Diffusion \\ 
FLATTEN~\citep{cong2023flatten} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkgreen}{\ding{51}} & Stable Diffusion \\ 
Fairy~\citep{wu2023fairy} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkgreen}{\ding{51}} & Stable Diffusion \\ 
ControlVideo~\citep{zhang2023controlvideo} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & ControlNet \\ 
CoDeF~\citep{ouyang2023codef} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & ControlNet \\ 
VideoSwap~\citep{gu2023videoswap} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & AnimateDiff  \\ 
UniEdit~\citep{bai2024uniedit} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkred}{\ding{55}} & \textcolor{darkgreen}{\ding{51}} & Any T2V Models\\ 
\midrule
\textbf{\model (Ours)} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkgreen}{\ding{51}} & Any I2V Models \\ 
\bottomrule
\end{tabular}}
\label{tab:baselines}
\end{table}
% \end{wraptable}
